Semantic Complete Scene Forecasting from a 4D Dynamic Point Cloud Sequence

We study a new problem of semantic complete scene forecasting (SCSF) in this work. Given a 4D dynamic point cloud sequence, our goal is to forecast the complete scene corresponding to the future next frame along with its semantic labels. To tackle this challenging problem, we properly model the synergetic relationship between future forecasting and semantic scene completion through a novel network named SCSFNet. SCSFNet leverages a hybrid geometric representation for high-resolution complete scene forecasting. To leverage multi-frame observation as well as the understanding of scene dynamics to ease the completion task, SCSFNet introduces an attention-based skip connection scheme. To ease the need to model occlusion variations and to better focus on the occluded part, SCSFNet utilizes auxiliary visibility grids to guide the forecasting task. To evaluate the effectiveness of SCSFNet, we conduct experiments on various benchmarks including two large-scale indoor benchmarks we contributed and the outdoor SemanticKITTI benchmark. Extensive experiments show SCSFNet outperforms baseline methods on multiple metrics by a large margin, and also prove the synergy between future forecasting and semantic scene completion.

==> tables/results.tex <==

%
\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table}[t]
\centering
\footnotesize
\tablestyle{2.5pt}{1.05}
\begin{tabularx}{1.0\linewidth}{lY|YYY}
    \toprule
    \multicolumn{1}{c}{Task} & \multicolumn{1}{c}{Prediction} & \multicolumn{3}{c}{Complete Prediction} \\
     & CD & CD & IOU & mIOU \\
    \midrule
    TLFPAD \cite{tlfpad} & 0.043 & - & - & - \\ %
    Occlusion4D(P) \cite{vanhoorick2022revealing} & 0.050 & - & - & - \\ %
    Occlusion4D(CP) \cite{vanhoorick2022revealing} & - & 0.129 & - & - \\ %
    Occlusion4D(SCP) \cite{vanhoorick2022revealing} & - & 0.093 & 23.0(11.6) & 12.7(7.4) \\ %
    \hline
    P & 0.051 & - & - & - \\
    CP & 0.039 & 0.032 & 42.3(26.6) & - \\
    SCP & 0.038 & 0.032 & 42.6(31.0) & 31.2(22.4) \\
    \bottomrule
\end{tabularx}
\vspace{-0.1cm}
\caption{\textbf{Results on IGPLAY dataset}. We report Chamfer Distance of point clouds(lower is better, the unit is square meter), IoU of low-resolution voxel grids(on the left) as well as high-resolution ones(on the right, in brackets), and mIoU of low-resolution voxel grids(on the left) as well as high-resolution ones(on the right, in brackets).}
\vspace{-0.3cm}
\label{tables:igplay}
\end{table}

\setlength{\tabcolsep}{2pt} 

%
%

\begin{table}[t]
\centering
\footnotesize
\tablestyle{2.5pt}{1.05}
\begin{tabularx}{1.0\linewidth}{lY|YYY}
    \toprule
    \multicolumn{1}{c}{Task} & \multicolumn{1}{c}{Prediction} & \multicolumn{3}{c}{Complete Prediction} \\
     & CD & CD & IOU & mIOU \\
    \midrule
    TLFPAD \cite{tlfpad} & 0.047 & - & - & - \\ %
    Occlusion4D(P) \cite{vanhoorick2022revealing} & 0.100 & - & - & - \\ %
    Occlusion4D(CP) \cite{vanhoorick2022revealing} & - & 0.113 & - & - \\ %
    Occlusion4D(SCP) \cite{vanhoorick2022revealing} & - & 0.138 & 49.2(41.3) & 23.5(18.9) \\ %
    \hline
    P & 0.038 & - & - & - \\
    CP & 0.034 & 0.028 & 66.8(50.2) & - \\
    SCP & 0.030 & 0.023 & 69.1(54.9) & 33.7(27.6) \\
    \bottomrule
\end{tabularx}
\vspace{-0.1cm}
\caption{\textbf{Results on IGNAV dataset}. We report Chamfer Distance of point clouds(lower is better, the unit is square meter), IoU of low-resolution voxel grids(on the left) as well as high-resolution ones(on the right, in brackets), and mIoU of low-resolution voxel grids(on the left) as well as high-resolution ones(on the right, in brackets).}\vspace{-0.4cm}
\label{tables:ignav}
\end{table}

==> tables/semanticKITTI.tex <==
\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table}[h]
\vspace{-0.41cm}
\centering
\footnotesize
\tablestyle{1.5pt}{1.05}
\begin{tabularx}{1.0\linewidth}{lY|YYY}
    \toprule
    \multicolumn{1}{c}{SemanticKITTI Task} & \multicolumn{1}{c}{Prediction} & \multicolumn{3}{c}{Complete Prediction} \\
     & CD & CD & IoU & mIoU \\
    \midrule
    % Occlusion4D(CSF)  & 3.00 & 4.37 & 39.1(16.7) & - \\ %
    Occlusion4D(SCSF) & 3.23 & 4.16 & 39.2(16.5) & 9.1(5.9) \\ %
    % \hline
    % CSF & 0.80 & 3.73 & 45.8(29.1) & - \\
    SCSF & 0.77 & 3.49 & 49.1(27.0) & 13.0(7.7) \\
    \bottomrule
\end{tabularx}
% \vspace{-0.1cm}
%\caption{\textbf{Results on SemanticKITTI dataset.}}
\vspace{-0.5cm}
\label{tables:semnaticKITTI}
\end{table}
